Annotated Stack Trees

Annotated pushdown automata provide an automaton model of higher-order recursion schemes, which may in turn be used to model higher-order programs for the purposes of verification. We study Ground Annotated Stack Tree Rewrite Systems -- a tree rewrite system where each node is labelled by the configuration of an annotated pushdown automaton. This allows the modelling of fork and join constructs in higher-order programs and is a generalisation of higher-order stack trees recently introduced by Penelle. We show that, given a regular set of annotated stack trees, the set of trees that can reach this set is also regular, and constructible in n-EXPTIME for an order-n system, which is optimal. We also show that our construction can be extended to allow a global state through which unrelated nodes of the tree may communicate, provided the number of communications is subject to a fixed bound.

==> context-bounding-icalp.tex <==

\section{Context Bounding}

In the model discussed so far, communication between different nodes of the tree
had to be done locally (i.e. from parent to child, via the destruction of
nodes).  In Appendix~\ref{sec:context-bounding}, we show that the saturation
algorithm can be extended to allow a bounded amount of communication between
distant nodes of the tree.  This communication is via a global control state
that can always be read, but only changed an \textit{a priori} fixed number of
times.

\begin{definition}
      [Order-$\maxord$ GASTRSs with Global State]
    An \emph{order-$\maxord$ GASTRS with global state} $\gstrs$ is a tuple
    $\tup{\salphabet, \controls, \globals, \rules}$
    where $\salphabet$ is a finite stack alphabet, $\controls$ is a finite set
    of control states, $\globals$ is a finite set of global states, and
    $\rules
     \subset
     \globals
     \times
     \stacktreeops{\maxord}{\salphabet}{\controls} \times \globals$
    is a finite set of operations.
\end{definition}

A configuration is a pair
$\config{\gstate}{\tree}$
where
$\gstate \in \globals$
and $\tree$ is an order-$\maxord$ annotated stack tree.  We have
$\config{\gstate}{\tree} \tran \config{\gstate'}{\tree'}$
whenever
$\tup{\gstate, \strule, \gstate'} \in \rules$
and
$\tree' \in \ap{\strule}{\tree}$.

We define and solve the context-bounded reachability problem formally in
Appendix~\ref{sec:context-bounding}.  Intuitively,
a run is context bounded for a bound $\lifespan$ if there are at most
$\lifespan$ changes to the control state that occur in the run.  The global
context-bounded backwards reachability problem is to construct the set of
configurations that may reach a given target set.  We obtain an algorithm for
this reachability problem by guessing the sequence of global control states
seen, and then performing a sequence of saturation steps, one for each control
state.

We begin with $\ta_0$.  A saturation step gives us the set of trees that
reach $\ta_0$ for a fixed $\gstate$.  Then, we update the saturated automaton
to reflect a single application in the tree of a rule that changes the global
state.  Applying another saturation step gives us the set of trees that run in
one global state, perform a state change, then run to $\ta_0$.  By iterating
this procedure, we solve the context-bounded reachability problem.

\begin{namedtheorem}{thm:context-bounded}{Context-Bounded Reachability}
    The global context-bounded backwards reachability problem for GASTRS with
    global state is decidable.
\end{namedtheorem}



==> correctness.tex <==

\section{Correctness of Saturation}
\label{sec:correctness}

We prove that saturation is correct and runs in $\maxord$-EXPTIME.

\begin{proof}[Proof of \refproperty{prop:sat-correct}]
    The proof of completeness is given in Lemma~\ref{lem:completeness} and
    soundness is given in Lemma~\ref{lem:soundness}.

    The complexity is derived as follows.  We add at most one transition of the
    form
    $\tatran{\tastate}{\idxi}{\numof}{\control}{\sastate}$
    for each $\tastate$, $\idxi$, $\numof$ and $\control$.  Hence we add at most
    a polynomial number of transitions to $\tadelta$.

    Thus, to $\sadelta_\maxord$ we have a polynomial number of states.  We add at
    most one transition of the form
    $\sastate \satran{\sastate'} \sastateset$
    for each $\sastate$ and set of states $\sastateset$.  Thus we have at most
    an exponential number of transitions in $\sadelta_\maxord$.

    Thus, in $\sastates_\midord$ we have a number of states bounded by a tower
    of exponentials of height
    $(\maxord - \midord)$.
    Since we add at most one transition of the form
    $\sastate \satran{\sastate'} \sastateset$
    for each $\sastate$ and $\sastateset$ we have a number of transitions
    bounded by a tower of exponentials of height
    $(\maxord - \midord + 1)$
    giving the number of states in
    $\sastates_{\midord-1}$.

    Thus, at order-$1$ the number of new transitions is bounded by a tower of
    height $\maxord$, giving the $\maxord$-EXPTIME complexity.
\end{proof}



